Fast emulation of anisotropies induced in the cosmic microwave background by cosmic strings

Cosmic strings are linear topological defects that may have been produced during symmetry-breaking phase transitions in the very early Universe. In an expanding Universe the existence of causally separate regions prevents such symmetries from being broken uniformly, with a network of cosmic string inevitably forming as a result. To faithfully generate observables of such processes requires computationally expensive numerical simulations, which prohibits many types of analyses. We propose a technique to instead rapidly emulate observables, thus circumventing simulation. Emulation is a form of generative modelling, often built upon a machine learning backbone. End-to-end emulation often fails due to high dimensionality and insufficient training data. Consequently, it is common to instead emulate a latent representation from which observables may readily be synthesised. Wavelet phase harmonics are an excellent latent representations for cosmological fields, both as a summary statistic and for emulation, since they do not require training and are highly sensitive to non-Gaussian information. Leveraging wavelet phase harmonics as a latent representation, we develop techniques to emulate string induced CMB anisotropies over a 7.2 degree field of view, with sub-arcminute resolution, in under a minute on a single GPU. Beyond generating high fidelity emulations, we provide a technique to ensure these observables are distributed correctly, providing a more representative ensemble of samples. The statistics of our emulations are commensurate with those calculated on comprehensive Nambu-Goto simulations. Our findings indicate these fast emulation approaches may be suitable for wide use in, e.g., simulation based inference pipelines. We make our code available to the community so that researchers may rapidly emulate cosmic string induced CMB anisotropies for their own analysis.

==> macros.tex <==
%==============================================================================
% Comments
%==============================================================================

\newcommand{\todo}[1]{\textcolor{red}{[{\bf TODO}: #1]}}
\newcommand{\jdm}[1]{\textcolor{red}{[{\bf JDM}: #1]}}


%==============================================================================
% Abbreviations
%==============================================================================

\newcommand{\eqn}[1]{(#1)}
\newcommand{\Eqn}[1]{(#1)}
\newcommand{\tbl}[1]{Table~#1}
\newcommand{\Tbl}[1]{Table~#1}
\newcommand{\fig}[1]{Fig.~#1}
\newcommand{\Fig}[1]{Fig.~#1}
\newcommand{\sectn}[1]{Sec.~#1}
\newcommand{\Sectn}[1]{Sec.~#1}
\newcommand{\chap}[1]{Chapter~#1}
\newcommand{\Chap}[1]{Chapter~#1}
\newcommand{\appn}[1]{Appendix~#1}
\newcommand{\Appn}[1]{Appendix~#1}
\newcommand{\lemmaref}[1]{Lemma~#1}

\newcommand{\etal}{\mbox{\it et al.}}
\newcommand{\eg}{\mbox{\it e.g.}}
\newcommand{\ie}{\mbox{\it i.e.}}
\newcommand{\etc}{\mbox{\it etc.}}
\newcommand{\cf}{\mbox{\it cf.}}


%==============================================================================
% Units
%==============================================================================

\newcommand{\ghz}{{GHz}}
\newcommand{\joule}{{J}}
\newcommand{\watt}{{W}}
\newcommand{\metre}{m}
\newcommand{\nanometre}{nm}
\newcommand{\steradian}{sr}
\newcommand{\kelvin}{{K}}
% \newcommand{\arcmin}{\ensuremath{{}^\prime}}
\newcommand{\degrees}{\ensuremath{{^\circ}}}


%==============================================================================
% Acronyms
%=============================================================================

\newcommand{\fft}{{FFT}}
\newcommand{\dft}{{DFT}}

\newcommand{\frw}{{FRW}}
\newcommand{\frwtext}{{Friedmann-Robertson-Walker}}

\newcommand{\cmb}{{CMB}}
\newcommand{\cmbtext}{{cosmic microwave background}}
\newcommand{\Cmbtext}{{Cosmic microwave background}}

\newcommand{\wmap}{{WMAP}}
\newcommand{\wmaptext}{{Wilkinson Microwave Anisotropy Probe}}
\newcommand{\ilc}{{ILC1}}
\newcommand{\ilcthree}{{ILC3}}
\newcommand{\ilctext}{{internal linear combination}}

\newcommand{\planck}{\textit{Planck}}

\newcommand{\cobedmr}{\mbox{COBE-DMR}}
\newcommand{\cobedmrtext}{Cosmic Background Explorer-Differential Microwave Radiometer}
\newcommand{\cobe}{\mbox{COBE}}

\newcommand{\bianchi}{{Bianchi}}
\newcommand{\bianchiviih}{{Bianchi VII{$_{\lowercase{h}}$}}}
\newcommand{\wmapbianchi}{{\wmap1$-$Bianchi}}

\newcommand{\isw}{{ISW}}
\newcommand{\iswtext}{{integrated Sachs-Wolfe}}
\newcommand{\Iswtext}{{Integrated Sachs-Wolfe}}

\newcommand{\cswt}{{CSWT}}
\newcommand{\cswti}{\mbox{CSWT$_{\rm I}$}}
\newcommand{\cswtii}{\mbox{CSWT$_{\rm II}$}}
\newcommand{\cswttext}{continuous spherical wavelet transform}
\newcommand{\Cswttext}{Continuous spherical wavelet transform}

\newcommand{\lss}{{LSS}}
\newcommand{\lsstext}{large scale structure}
\newcommand{\Lsstext}{Large scale structure}

\newcommand{\nvss}{{NVSS}}
\newcommand{\nvsstext}{{NRAO VLA Sky Survey}}

\newcommand{\sdss}{{SDSS}}
\newcommand{\sdsstext}{Sloan Digital Sky Survey}

\newcommand{\twomass}{{2MASS}}
\newcommand{\twomasstext}{Two Micron All Sky Survey}

\newcommand{\lcdm}{\ensuremath{\Lambda}{CDM}}
\newcommand{\lcdmtext}{\ensuremath{\Lambda} Cold Dark Matter}

\newcommand{\ska}{{SKA}}
\newcommand{\skatext}{Square Kilometre Array}

\newcommand{\smhwtext}{{spherical Mexican hat wavelet}}
\newcommand{\smhw}{{SMHW}}
\newcommand{\semhw}{{SEMHW}}
\newcommand{\smw}{{SMW}}
\newcommand{\sbwtext}{{spherical butterfly wavelet}}
\newcommand{\sbw}{{SBW}}
\newcommand{\mexhat}{Mexican hat}
\newcommand{\Mexhat}{Mexican hat}
\newcommand{\morlet}{real Morlet}
\newcommand{\Morlet}{Real Morlet}

\newcommand{\healpix}{{\tt HEALPix}}
\newcommand{\healpixtext}{{Hierarchical Equal Area isoLatitude Pixelisation of the sphere}}
\newcommand{\cmbfast}{\mbox{\tt CMBFAST}}
\newcommand{\camb}{\mbox{\tt CAMB}}
\newcommand{\cosmomc}{\mbox{\tt COSMOMC}}
\newcommand{\anicosmo}{\mbox{\tt ANICOSMO}}

\newcommand{\yawtbtext}{{Yet Another Wavelet Toolbox}}
\newcommand{\yawtb}{{\tt YAWTb}}

\newcommand{\stwo}{{\tt S2}}
\newcommand{\stwofil}{{\tt S2FIL}}
\newcommand{\fastcswt}{{\tt FastCSWT}}
\newcommand{\comb}{{\tt COMB}}
\newcommand{\bianchicode}{{\tt Bianchi}}
\newcommand{\bianchicodetwo}{{\tt Bianchi2}}
\newcommand{\sshtcode}{{\tt SSHT}}
\newcommand{\sothreecode}{{\tt SO3}}
\newcommand{\stwoletcode}{{\tt S2LET}}

\newcommand{\lambdaarch}{{LAMBDA}}
\newcommand{\lambdaarchtext}{{Legacy Archive for Microwave Background Data Analysis}}

\newcommand{\kpzero}{{Kp0}}
\newcommand{\tohmap}{{TOH}}

\newcommand{\fwhm}{{FWHM}}
\newcommand{\fwhmtext}{{full-width-half-maximum}}
\newcommand{\snr}{{\rm SNR}}
\newcommand{\snrp}{\ensuremath{\snr_{\pind}}}
\newcommand{\snrs}{\ensuremath{\snr_{\sind}}}

\newcommand{\mf}{{MF}}
\newcommand{\saf}{{SAF}}

\newcommand{\fov}{FOV}
\newcommand{\wfov}{WFOV}
\newcommand{\wterm}{\mbox{$w$-term}}


%==============================================================================
% Data
%==============================================================================

\newcommand{\spotloc}{\mbox{\ensuremath{(l,b)=(209^\circ,-57^\circ)}}}


%==============================================================================
% Maths
%==============================================================================

% General
\newcommand{\spcend}{\ensuremath{\:}}
\newcommand{\img}{\ensuremath{{\rm i}}}
\newcommand{\cconj}{\ensuremath{\ast}} 
\newcommand{\adjoint}{\ensuremath{{}^\dagger}} 
\newcommand{\reals}{\ensuremath{\mathbb{R}}}
\newcommand{\realsnn}{\ensuremath{\mathbb{R^+}}}
\newcommand{\realsnz}{\ensuremath{\mathbb{R}^{+}_{\ast}}}
\newcommand{\integers}{\ensuremath{\mathbb{Z}}}
\newcommand{\naturals}{\ensuremath{\mathbb{N}}}
\newcommand{\complex}{\ensuremath{\mathbb{C}}}
\newcommand{\ltwo}{\ensuremath{\mathrm{L}^2}}
\newcommand{\sphere}{\ensuremath{{\mathbb{S}^2}}}
\newcommand{\sothree}{\ensuremath{{\mathrm{SO}(3)}}}
\newcommand{\sotwo}{\ensuremath{{\mathrm{SO}(2)}}}
\newcommand{\torus}{\ensuremath{{\mathrm{T}^2}}}
\newcommand{\disk}{\ensuremath{{D^2}}}
\newcommand{\ball}{{\ensuremath{\mathbb{B}^3}}}
\newcommand{\ipball}{\ensuremath{\ball}}
\newcommand{\ipsphere}{\ensuremath{\sphere}}
\newcommand{\iphalfline}{\ensuremath{\realsnn}}
\newcommand{\vect}[1]{\ensuremath{\mbox{\boldmath ${#1}$}}}
\newcommand{\vectsm}[1]{\ensuremath{\mbox{\boldmath \footnotesize ${#1}$}}}
\newcommand{\xvect}{\vect{x}}
\newcommand{\kvect}{\vect{k}}
\newcommand{\zerovect}{\ensuremath{\mathbf{0}}}
\newcommand{\knaut}{\ensuremath{k_0}}
\newcommand{\nsigma}{\ensuremath{N_\sigma}}
\newcommand{\zreal}{{\ensuremath{\rm{Re}}}}
\newcommand{\zimag}{{\ensuremath{\rm{Im}}}}
\newcommand{\dotprod}{\ensuremath{\cdot}}
\newcommand{\likelihood}{\ensuremath{\mathcal{L}}}
\newcommand{\prior}{\ensuremath{\pi}}
% \newcommand{\evidence}{\ensuremath{Z}}
\newcommand{\opnexpv}{\ensuremath{\langle}}
\newcommand{\clsexpv}{\ensuremath{\rangle}}

% Integrals
\newcommand{\dx}{\ensuremath{\mathrm{\,d}}}
\newcommand{\dmu}[1]{\ensuremath{\dx \Omega(#1)}}
\newcommand{\dmun}{\ensuremath{\dx \Omega}}
\newcommand{\deul}[1]{\ensuremath{\dx \varrho(#1)}}
\newcommand{\deuln}{\ensuremath{\dx \varrho}}
\newcommand{\ddr}{\ensuremath{\frac{\partial}{\partial\scale}}}
\newcommand{\innerp}[2]{\ensuremath{\langle {#1},\: {#2} \rangle}}

% Theorems
% \theoremstyle{remark}
% \newtheorem{lemma}{Lemma}[section]
% \theoremstyle{plain}
% \newtheorem{result}{Result}
% \theoremstyle{definition}
% \newtheorem*{definition}{Definition}
% \newcommand{\thmend}{{\mbox{}  \hfill \raggedright \ensuremath{\blacksquare}\\[3mm]}}

% Physics of the universe
\newcommand{\clight}{\ensuremath{c}}
\newcommand{\ctime}{\ensuremath{\eta}}
\newcommand{\ptime}{\ensuremath{t}}
\newcommand{\pdist}{\ensuremath{d}}
\newcommand{\rvel}{\ensuremath{v}}
\newcommand{\hub}{\ensuremath{H}}
\newcommand{\hubsmall}{\ensuremath{h}}
\newcommand{\scfac}{\ensuremath{R}}
\newcommand{\scfacd}{\ensuremath{\dot{\scfac}}}
\newcommand{\scfacdd}{\ensuremath{\ddot{\scfac}}}
\newcommand{\kcurv}{\ensuremath{k}}
\newcommand{\cconst}{\ensuremath{\Lambda}}
\newcommand{\gconst}{\ensuremath{G}}
\newcommand{\den}{\ensuremath{\rho}}
\newcommand{\denmat}{\ensuremath{\rho_{\rm m}}}
\newcommand{\denrad}{\ensuremath{\rho_{\rm r}}}
\newcommand{\dencrit}{\ensuremath{\rho_{\rm c}}}
\newcommand{\Den}{\ensuremath{\Omega}}
\newcommand{\Dentot}{\ensuremath{\Den_{\rm total}}}
\newcommand{\Denmat}{\ensuremath{\Den_{\rm m}}}
\newcommand{\Denmatc}{\ensuremath{\Den_{\rm c}}}
\newcommand{\Denmatb}{\ensuremath{\Den_{\rm b}}}
\newcommand{\Dencurvature}{\ensuremath{\Den_{k}}}
\newcommand{\Denrad}{\ensuremath{\Den_{\rm r}}}
\newcommand{\Denlambda}{\ensuremath{\Den_{\Lambda}}}
\newcommand{\pres}{\ensuremath{p}}
\newcommand{\w}{\ensuremath{w}}
\newcommand{\z}{\ensuremath{z}}
\newcommand{\zrec}{\ensuremath{\z_{\rm rec}}}

% CMB
\newcommand{\dtemp}{\ensuremath{\Delta T}}
\newcommand{\temp}{\ensuremath{T_0}}
\newcommand{\rdtemp}{\ensuremath{\frac{\dtemp}{\temp}}}
\newcommand{\gravpotent}{\ensuremath{\delta\Phi}}
\newcommand{\cl}{\ensuremath{C_\el}}
\newcommand{\clest}{\ensuremath{\widehat{C}_\el}}

% Variables (e.g. spherical coordinates, indices, scales)
\newcommand{\sa}{\ensuremath{\omega}}
\newcommand{\saa}{\ensuremath{\theta}}
\newcommand{\sab}{\ensuremath{\varphi}}
\newcommand{\sas}{\ensuremath{\saa, \sab}}
\newcommand{\radvec}{\ensuremath{\vect{\rad}}}
\newcommand{\radvecunit}{\ensuremath{\hat{\vect{\rad}}}}
\newcommand{\eul}{\ensuremath{\mathbf{\rho}}}
\newcommand{\euls}{\ensuremath{\eula, \eulb, \eulc}}
\newcommand{\eula}{\ensuremath{\alpha}}
\newcommand{\eulb}{\ensuremath{\beta}}
\newcommand{\eulc}{\ensuremath{\gamma}}
\newcommand{\eulai}{\ensuremath{a}}
\newcommand{\eulbi}{\ensuremath{b}}
\newcommand{\eulci}{\ensuremath{g}}
\newcommand{\eulaiang}{\ensuremath{\eula_\eulai}}
\newcommand{\eulbiang}{\ensuremath{\eulb_\eulbi}}
\newcommand{\eulciang}{\ensuremath{\eulc_\eulci}}
\newcommand{\el}{\ensuremath{\ell}}
\newcommand{\m}{\ensuremath{m}}
\newcommand{\n}{\ensuremath{n}}
\newcommand{\ip}{\ensuremath{p}}
\newcommand{\spin}{\ensuremath{s}}
\newcommand{\elm}{\ensuremath{{\el\m}}}
\newcommand{\elp}{\ensuremath{{\el\p}}}
\newcommand{\elmax}{\ensuremath{{L}}}
%\newcommand{\mmax}{\ensuremath{\m_{\rm max}}}
\newcommand{\mmax}{\ensuremath{{M}}}
\newcommand{\nmax}{\ensuremath{{N}}}
\newcommand{\ipmax}{\ensuremath{{P}}}
\newcommand{\p}{\ensuremath{^\prime}}
\newcommand{\pp}{\ensuremath{^{\prime\prime}}}
\newcommand{\scale}{\ensuremath{R}}
\newcommand{\scalenaut}{\ensuremath{R_0}}
\newcommand{\scalea}{\ensuremath{a}}
\newcommand{\scaleb}{\ensuremath{b}}
\newcommand{\scaleab}{\ensuremath{{\scalea,\scaleb}}}
\newcommand{\rad}{\ensuremath{r}}
\newcommand{\cmbtemp}{\ensuremath{T}}
\newcommand{\pixw}{\ensuremath{p_\el}}
%\newcommand{\bm}[1]{\ensuremath{b_\el^{#1}}}
\newcommand{\pind}{\ensuremath{{\rm p}}}
\newcommand{\sind}{\ensuremath{{\rm s}}}
\newcommand{\mind}{\ensuremath{{m}}}
\newcommand{\tfov}{\ensuremath{\saa_{\rm \fov}}}

% Coordinate systems
\newcommand{\nind}{\ensuremath{\hat{\vect{n}}_i}}
\newcommand{\none}{\ensuremath{\hat{\vect{n}}_1}}
\newcommand{\ntwo}{\ensuremath{\hat{\vect{n}}_2}}
\newcommand{\nthree}{\ensuremath{\hat{\vect{n}}_3}}
\newcommand{\gind}{\ensuremath{\hat{\vect{g}}_i}}
\newcommand{\gone}{\ensuremath{\hat{\vect{g}}_1}}
\newcommand{\gtwo}{\ensuremath{\hat{\vect{g}}_2}}
\newcommand{\gthree}{\ensuremath{\hat{\vect{g}}_3}}
\newcommand{\eind}{\ensuremath{\hat{\vect{e}}_i}}
\newcommand{\eone}{\ensuremath{\hat{\vect{e}}_1}}
\newcommand{\etwo}{\ensuremath{\hat{\vect{e}}_2}}
\newcommand{\ethree}{\ensuremath{\hat{\vect{e}}_3}}
\newcommand{\uone}{\ensuremath{\hat{\vect{u}}_1}}
\newcommand{\utwo}{\ensuremath{\hat{\vect{u}}_2}}
\newcommand{\uthree}{\ensuremath{\hat{\vect{u}}_3}}

% Special functions and harmonic coefficients
\newcommand{\kron}[2]{\ensuremath{\delta_{{#1}{#2}}}}
\newcommand{\kronsp}[2]{\ensuremath{\delta_{{#1},{#2}}}}
\newcommand{\dirac}{\ensuremath{\delta}}
\newcommand{\poly}{\ensuremath{\phi}}
\newcommand{\polyw}{\ensuremath{w}}
\renewcommand{\exp}[1]{\ensuremath{{\rm e}^{#1}}}
\newcommand{\shfarg}[3]{\ensuremath{Y_{#1#2}({#3})}}
\newcommand{\shfargc}[3]{\ensuremath{Y_{#1#2}^\cconj({#3})}}
\newcommand{\shfargsp}[3]{\ensuremath{Y_{{#1},{#2}}({#3})}}
\newcommand{\sshfarg}[4]{\ensuremath{{{}_{#4} Y_{#1#2}({#3})}}}
\newcommand{\sshfargc}[4]{\ensuremath{{{}_{#4} Y_{#1#2}^\cconj({#3})}}}
\newcommand{\sshfargsp}[4]{\ensuremath{{{}_{#4} Y_{{#1},{#2}}({#3})}}}
\newcommand{\shf}[2]{\ensuremath{Y_{#1#2}}}
\newcommand{\shfc}[2]{\ensuremath{Y_{#1#2}^\cconj}}
\newcommand{\shc}[3]{\ensuremath{{#1}_{{#2}{#3}}}}
\newcommand{\shcc}[3]{\ensuremath{{#1}_{{#2}{#3}}^\cconj}}
\newcommand{\shcsp}[3]{\ensuremath{{#1}_{{#2},{#3}}}}
\newcommand{\shccsp}[3]{\ensuremath{{#1}_{{#2},{#3}}^\cconj}}
\newcommand{\sshf}[3]{\ensuremath{{\prescript{}{#3} Y_{#1#2}}}}
\newcommand{\sshfc}[3]{\ensuremath{{\prescript{}{#3} Y_{#1#2}^\cconj}}}
\newcommand{\sshc}[4]{\ensuremath{\prescript{}{#4} {#1}_{{#2}{#3}}}}
\newcommand{\sshcc}[4]{\ensuremath{\prescript{}{#4} {#1}_{{#2}{#3}}^\cconj}}
\newcommand{\sshcsp}[4]{\ensuremath{\prescript{}{#4} {#1}_{{#2},{#3}}}}
\newcommand{\sshccsp}[4]{\ensuremath{\prescript{}{#4} {#1}_{{#2},{#3}}^\cconj}}
\newcommand{\leg}[2]{\ensuremath{P_{{#1}}({#2})}}
\newcommand{\aleg}[3]{\ensuremath{P_{#1}^{#2}({#3})}}
\newcommand{\legc}[2]{\ensuremath{{#1}_{#2}}}
\newcommand{\daleg}[3]{\ensuremath{P_{#1}^{#2\prime}({#3})}}
\newcommand{\sbessel}[1]{\ensuremath{j_{#1}}}
\newcommand{\bessel}[2]{\ensuremath{J_{#1}({#2})}}
\newcommand{\jacobi}[4]{\ensuremath{P_{#1}^{(#2,#3)}({#4})}}
\newcommand{\jacobia}{\ensuremath{a}}
\newcommand{\jacobib}{\ensuremath{b}}
\newcommand{\gammafun}{\ensuremath{\Gamma}}
% \newcommand{\binomial}[2]{\ensuremath{\left( \begin{array}{c} {#1} \\ {#2} \end{array} \right)}}
\newcommand{\binomial}[2]{\ensuremath{\,\, {}^{#1} C_{#2} \,\,}}

% Wigner functions
\newcommand{\dmatbig}{\ensuremath{D}}
\newcommand{\Dlmn}{\ensuremath{ \dmatbig_{\m\n}^{\el} }}
\newcommand{\Dlmnc}{\ensuremath{ \dmatbig_{\m\n}^{\el\cconj} }}
\newcommand{\Dlmz}{\ensuremath{ \dmatbig_{\m0}^{\el} }}
\newcommand{\Dlmzc}{\ensuremath{ \dmatbig_{\m0}^{\el\cconj} }}
\newcommand{\Dlmnp}{\ensuremath{ \dmatbig_{\m\n}^{\el}(\eul) }}
\newcommand{\Dlmnpc}{\ensuremath{ \dmatbig_{\m\n}^{\el\cconj}(\eul) }}
\newcommand{\Dlmnabg}{\ensuremath{ \dmatbig_{\m\n}^{\el}(\euls) }}
\newcommand{\Dlmnabgc}{\ensuremath{ \dmatbig_{\m\n}^{\el\cconj}(\euls) }}
\newcommand{\dmatsmall}{\ensuremath{d}}
\newcommand{\dlmn}{\ensuremath{ \dmatsmall_{\m\n}^{\el} }}
\newcommand{\dlmnc}{\ensuremath{ \dmatsmall_{\m\n}^{\el\cconj} }}
\newcommand{\dlnm}{\ensuremath{ \dmatsmall_{\n\m}^{\el} }}
\newcommand{\dlmz}{\ensuremath{ \dmatsmall_{\m0}^{\el} }}
\newcommand{\dlmzc}{\ensuremath{ \dmatsmall_{\m0}^{\el\cconj} }}
\newcommand{\dlmnb}{\ensuremath{ \dmatsmall_{\m\n}^{\el}(\eulb) }}
\newcommand{\dlmnbc}{\ensuremath{ \dmatsmall_{\m\n}^{\el\cconj}(\eulb) }}
\newcommand{\dlnmb}{\ensuremath{ \dmatsmall_{\n\m}^{\el}(\eulb) }}
\newcommand{\dlmnhalfpi}[3]{\ensuremath{ \Delta_{{#2}{#3}}^{#1} }}
\newcommand{\dlmnhalfpic}[3]{\ensuremath{ \Delta_{{#2},{#3}}^{#1} }}
\newcommand{\dlmnhalfpim}{\ensuremath{ \Delta_{{\m\p}{\m}}^{\el} }}
\newcommand{\dlmnhalfpin}{\ensuremath{ \Delta_{{\m\p}{\n}}^{\el} }}
\newcommand{\dlmnhalfpisn}{\ensuremath{ \Delta_{{\m\p}{,-\spin}}^{\el} }}
\newcommand{\wigc}[4]{\ensuremath{{#1}^{#2}_{{#3}{#4}}}}

% Operators (e.g. rotations and dilations)
\newcommand{\dil}{\ensuremath{\mathcal{D}}}
\newcommand{\dilsmall}{\ensuremath{d}}
\newcommand{\spo}{\ensuremath{\Pi}}
\newcommand{\rot}{\ensuremath{\mathcal{R}}}
\newcommand{\rotarg}[1]{\ensuremath{\mathcal{R}_{#1}}}
\newcommand{\rotmat}{\ensuremath{\mathbf{\mathsf{R}}}}
\newcommand{\rotmatarg}[1]{\ensuremath{\rotmat_{#1}}}
\newcommand{\transl}{\ensuremath{\mathcal{T}}}
\newcommand{\spinup}{\ensuremath{\eth}}
\newcommand{\spindown}{\ensuremath{\bar{\eth}}}

% Spherical wavelets
\newcommand{\sky}{\ensuremath{f}}
\newcommand{\f}{\ensuremath{f}}
% \newcommand{\fs}{\ensuremath{{}_\spin f}}
% \newcommand{\fsm}{\ensuremath{{{}_{-\spin} f}}}
% \newcommand{\flm}{\ensuremath{\shc{\f}{\el}{\m}}}
% \newcommand{\fslm}{\ensuremath{\shc{\fs}{\el}{\m}}}
\newcommand{\skywav}{\ensuremath{{\mathcal{W}_\wav^\sky}}}
\newcommand{\skywavni}{\ensuremath{{\mathcal{W}}}}
\newcommand{\skywavi}{\ensuremath{{\widehat{\mathcal{W}}_\wavi^\sky}}}
\newcommand{\skyLwavii}{\ensuremath{{\widetilde{\mathcal{W}}_\wavm^{\Lopii\sky}}}}
\newcommand{\skywavii}{\ensuremath{{\widetilde{\mathcal{W}}_\wavm^\sky}}}
\newcommand{\wavop}{\ensuremath{\mathcal{W}}}
\newcommand{\wav}{\ensuremath{\psi}}
\newcommand{\swav}{\ensuremath{{}_\spin\psi}}
\newcommand{\wavi}{\ensuremath{\Phi}}
\newcommand{\wavii}{\ensuremath{\Psi}}
\newcommand{\wavm}{\ensuremath{\Upsilon}}
\newcommand{\wavmc}{\ensuremath{\Upsilon^\cconj}}
\newcommand{\wavs}{\ensuremath{\Phi}}
\newcommand{\swavs}{\ensuremath{{}_\spin\Phi}}
\newcommand{\wcoeff}{\ensuremath{W}}
\newcommand{\scoeff}{\ensuremath{W}}
\newcommand{\wscale}{\ensuremath{j}}
\newcommand{\wscalemax}{\ensuremath{J}}
\newcommand{\wscalemin}{\ensuremath{J_0}}
\newcommand{\wposn}{\ensuremath{\eul}}
\newcommand{\wscaleposn}{\ensuremath{{\wscale\wposn}}}
\newcommand{\dilparam}{\ensuremath{\alpha}}
\newcommand{\wavker}{\ensuremath{\kappa}}
\newcommand{\wavsteer}{\ensuremath{\zeta}}
\newcommand{\steerinterp}{\ensuremath{z}}
\newcommand{\admissC}{\ensuremath{C}}
\newcommand{\admissCi}{\ensuremath{\widehat{\admissC}_\wavi}}
\newcommand{\admissCli}{\ensuremath{\widehat{\admissC}_\wavi^\el}}
\newcommand{\admissCii}{\ensuremath{\widetilde{\admissC}_\wavm}}
\newcommand{\admissClii}{\ensuremath{\widetilde{\admissC}_\wavm^\el}}
\newcommand{\Lopi}{\ensuremath{\widehat{L}_\wavi}}
\newcommand{\Lopii}{\ensuremath{\widetilde{L}_\wavm}}
\newcommand{\cocycle}{\ensuremath{\lambda}}
\newcommand{\effsize}{\ensuremath{\xi}}
\newcommand{\eccen}{\ensuremath{\epsilon}}
\newcommand{\sigx}{\ensuremath{\sigma_x}}
\newcommand{\sigy}{\ensuremath{\sigma_y}}

% Radon and ridgelet transforms
\newcommand{\sradon}{\ensuremath{\mathcal{S}}}
\newcommand{\sradondelta}{\ensuremath{\xi}}
\newcommand{\rwav}{\ensuremath{\psi}}
\newcommand{\srwav}{\ensuremath{{}_\spin\psi}}
\newcommand{\rwavs}{\ensuremath{\phi}}
\newcommand{\srwavs}{\ensuremath{{}_\spin\phi}}


\newcommand{\rwcoeff}{\ensuremath{G}}
\newcommand{\rscoeff}{\ensuremath{R}}
\newcommand{\rwavop}{\ensuremath{\mathcal{G}}}

% Common sums and fractions
\newcommand{\elmfact}{\ensuremath{\frac{(\el-\m)!}{(\el+\m)!}}}
\newcommand{\elpifrac}{\ensuremath{\frac{2\el+1}{4\pi}}}
\newcommand{\elpifracinv}{\ensuremath{\frac{4\pi}{2\el+1}}}
\newcommand{\sumlm}{\ensuremath{\sum_{\el=0}^{\infty} \sum_{\m=-\el}^\el}}
\newcommand{\sumlmn}{\ensuremath{\sum_{\el=0}^{\infty} \sum_{\m=-\el}^\el} \sum_{\n=-\el}^\el}
\newcommand{\suml}{\ensuremath{\sum_{\el=0}^{\infty}}}
\newcommand{\sumlmbl}{\ensuremath{\sum_{\el=0}^{\elmax-1} \sum_{\m=-\el}^\el}}
\newcommand{\sumlmnbl}{\ensuremath{\sum_{\el=0}^{\elmax-1} \sum_{\m=-\el}^\el} \sum_{\n=-\el}^\el}
\newcommand{\sumlbl}{\ensuremath{\sum_{\el=0}^{\elmax-1}}}
\newcommand{\summ}{\ensuremath{\sum_{\m=-\el}^\el}}
\newcommand{\summp}{\ensuremath{\sum_{\m\p=-\el}^\el}}
\newcommand{\sumn}{\ensuremath{\sum_{\n=-\el}^\el}}
\newcommand{\sumulm}{\ensuremath{\sum_{\el\m}}}
\newcommand{\sumulmn}{\ensuremath{\sum_{\el\m\n}}}
\newcommand{\sumlmp}{{\ensuremath{\sum_{\el\p =0}^{\infty} \: \sum_{\m\p=-\el\p }^{\el\p } \:}}}
\newcommand{\sumllm}{{\ensuremath{\sum_{\el =0}^{\infty} \: \sum_{\el\p =0}^{\infty} \: \sum_{\m\p=-\el }^{\el } \:}}}
\newcommand{\sumlmb}{\ensuremath{\sum_{\el \m}}}
\newcommand{\sumlmpb}{\ensuremath{\sum_{\elp \m\p}}}
\newcommand{\nl}{\ensuremath{\sqrt{\frac{2\el+1}{4\pi}}}}
\newcommand{\nlm}{\ensuremath{\sqrt{\frac{2\el+1}{4\pi}\frac{(\el-\m)!}{(\el+\m)!}}}}
\newcommand{\nlpmp}{\ensuremath{\sqrt{\frac{2\el\p+1}{4\pi}\frac{(\el\p-\m\p)!}{(\el\p+\m\p)!}}}}
\newcommand{\nlpm}{\ensuremath{\sqrt{\frac{2\el\p+1}{4\pi}\frac{(\el\p-\m)!}{(\el\p+\m)!}}}}

% Fast spin spherical harmonic transform
\newcommand{\G}[3]{\ensuremath{{{}_{#1} G_{{#2} {#3}}}}}
\newcommand{\Gtilde}[3]{\ensuremath{{{}_{#1} \tilde{G}_{{#2} {#3}}}}}
\newcommand{\rG}[3]{\ensuremath{{{}_{#1} \tilde{G}_{{#2} {#3}}}}}
\newcommand{\Gsm}{\ensuremath{\G{\spin}{\m}{}}}
\newcommand{\Gsmm}{\ensuremath{\G{\spin}{\m}{\m\p}}}
\newcommand{\Gsmt}{\ensuremath{\G{\spin}{\m}{}(\saa)}}
\newcommand{\rGsmt}{\ensuremath{\rG{\spin}{\m}{}(\saa)}}
\newcommand{\rGsmtn}{\ensuremath{\rG{\spin}{\m}{}(-\saa)}}
\newcommand{\Gsmti}{\ensuremath{\G{\spin}{\m}{}({\saaiang})}}
\newcommand{\Gsmtin}{\ensuremath{\G{\spin}{\m}{}({-\saaiang})}}
\newcommand{\rGsmti}{\ensuremath{\rG{\spin}{\m}{}({\saaiang})}}
\newcommand{\Gmn}{\ensuremath{G_{\m\n}}}
\newcommand{\Gmnm}{\ensuremath{G_{\m\n\m\p}}}
\newcommand{\Gmnb}{\ensuremath{G_{\m\n}(\eulb)}}
\newcommand{\Gmnbi}{\ensuremath{G_{\m\n}(\eulbiang)}}
\newcommand{\rGmnb}{\ensuremath{\tilde{G}_{\m\n}(\eulb)}}
\newcommand{\rGmnbi}{\ensuremath{\tilde{G}_{\m\n}(\eulbiang)}}
\newcommand{\Fmnm}{\ensuremath{\tilde{G}_{\m\n\m\p}}}
\newcommand{\Fmnmp}{\ensuremath{\tilde{G}_{\m\n\m\p{}\p}}}
\newcommand{\FImnm}{\ensuremath{F_{\m\n\m\p}}}
\newcommand{\F}[3]{\ensuremath{{{}_{#1} F_{{#2} {#3}}}}}
\newcommand{\rF}[3]{\ensuremath{{{}_{#1} \tilde{F}_{{#2} {#3}}}}}
\newcommand{\Fsm}{\ensuremath{\F{\spin}{\m}{}}}
\newcommand{\rFsm}{\ensuremath{\rF{\spin}{\m}{}}}
\newcommand{\Fsmm}{\ensuremath{\F{\spin}{\m}{\m\p}}}
\newcommand{\Fzmm}{\ensuremath{\F{0}{\m}{\m\p}}}
\newcommand{\Fsmmn}{\ensuremath{\F{\spin}{\m}{,-\m\p}}}
\newcommand{\Fsmnmn}{\ensuremath{\F{\spin}{-\m}{,-\m\p}}}
\newcommand{\Fzmmn}{\ensuremath{\F{0}{\m}{,-\m\p}}}
\newcommand{\Fzmnmn}{\ensuremath{\F{0}{-\m}{,-\m\p}}}
\newcommand{\Fsmmp}{\ensuremath{\F{\spin}{\m}{\m{\p}{\p}}}}
\newcommand{\Fsmt}{\ensuremath{\F{\spin}{\m}{}(\saa)}}
\newcommand{\rFsmt}{\ensuremath{\rF{\spin}{\m}{}(\saa)}}
\newcommand{\Fsmtn}{\ensuremath{\F{\spin}{\m}{}(-\saa)}}
\newcommand{\Fsmpt}{\ensuremath{\F{\spin}{\m\p}{}(\saa)}}
\newcommand{\intsaa}{\ensuremath{\int_0^{\pi} \dx \saa \sin \saa}}
\newcommand{\intsab}{\ensuremath{\int_0^{2\pi} \dx \sab}}
\newcommand{\saai}{\ensuremath{t}}
\newcommand{\sabi}{\ensuremath{p}}
\newcommand{\saaiang}{\ensuremath{\saa_\saai}}
\newcommand{\sabiang}{\ensuremath{\sab_\sabi}}
\newcommand{\sais}{\ensuremath{\sabi,\saai}}
\newcommand{\saisang}{\ensuremath{\saaiang,\sabiang}}
\newcommand{\sumsaai}{\ensuremath{\sum_{\saai=-(\elmax-1)}^{\elmax-1}}}
\newcommand{\sumsabi}{\ensuremath{\sum_{\sabi=-(\elmax-1)}^{\elmax-1}}}
\newcommand{\sumltrunc}{\ensuremath{\sum_{\el=0}^{\elmax-1}}}
\newcommand{\summtrunc}{\ensuremath{\sum_{\m=-(\elmax-1)}^{\elmax-1}}}
\newcommand{\summptrunc}{\ensuremath{\sum_{\m\p=-(\elmax-1)}^{\elmax-1}}}
\newcommand{\qweight}{\ensuremath{q}}
\newcommand{\qweightdh}{\ensuremath{\qweight_{\rm DH}}}
\newcommand{\qweightmw}{\ensuremath{\qweight_{\rm MW}}}
\newcommand{\weighttrans}{\ensuremath{v}}


% CMB polarisation
\newcommand{\stokesi}{\ensuremath{I}}
\newcommand{\stokesq}{\ensuremath{Q}}
\newcommand{\stokesu}{\ensuremath{U}}
\newcommand{\stokesv}{\ensuremath{V}}
\newcommand{\emode}{\ensuremath{E}}
\newcommand{\bmode}{\ensuremath{B}}
\newcommand{\emodetilde}{\ensuremath{\tilde{E}}}
\newcommand{\bmodetilde}{\ensuremath{\tilde{B}}}
\newcommand{\qpmiu}{\ensuremath{\stokesq \pm \img \stokesu}}
\newcommand{\qpiu}{\ensuremath{\stokesq + \img \stokesu}}
\newcommand{\qmiu}{\ensuremath{\stokesq - \img \stokesu}}


% Numerics
\newcommand{\cswtfftterm}{\ensuremath{T}}
\newcommand{\grideula}{\ensuremath{\mathcal{E}_1}}
\newcommand{\grideulb}{\ensuremath{\mathcal{E}_2}}
\newcommand{\gridhpix}{\ensuremath{\mathcal{H}}}
\newcommand{\gridecp}{\ensuremath{\mathcal{C}}}
\newcommand{\ia}{\ensuremath{{n_\eula}}}
\newcommand{\ib}{\ensuremath{{n_\eulb}}}
\newcommand{\ig}{\ensuremath{{n_\eulc}}}
\newcommand{\ik}{\ensuremath{{k}}}
\newcommand{\ith}{\ensuremath{{n_\saa}}}
\newcommand{\iph}{\ensuremath{{n_\sab}}}
\newcommand{\ipix}{\ensuremath{{p}}}
\newcommand{\na}{\ensuremath{{N_\eula}}}
\newcommand{\nb}{\ensuremath{{N_\eulb}}}
\newcommand{\ngm}{\ensuremath{{N_\eulc}}}
\newcommand{\nth}{\ensuremath{{N_\saa}}}
\newcommand{\nph}{\ensuremath{{N_\sab}}}
\newcommand{\N}{\ensuremath{{N}}}
\newcommand{\Ngl}{\ensuremath{{N_{\rm GL}}}}
\newcommand{\Ndh}{\ensuremath{{N_{\rm DH}}}}
\newcommand{\Nhw}{\ensuremath{{N_{\rm HW}}}}
\newcommand{\Nmw}{\ensuremath{{N_{\rm MW}}}}
\newcommand{\Nm}{\ensuremath{{N_{\rm M}}}}
\newcommand{\Ns}{\ensuremath{{N_{\rm S}}}}
\newcommand{\nside}{\ensuremath{{N_{\rm{side}}}}}
\newcommand{\npix}{\ensuremath{{N_{\rm{pix}}}}}
\newcommand{\pixarea}{\ensuremath{{\Omega_{\rm{pix}}}}}
\newcommand{\nplane}{\ensuremath{{N_{\pind}}}}
\newcommand{\nsphere}{\ensuremath{{N_{\sind}}}}
\newcommand{\weight}{\ensuremath{w}}
\newcommand{\order}{\ensuremath{\mathcal{O}}}

% Skewness and kurtosis related variables
\newcommand{\mean}{\ensuremath{\mu}}
\newcommand{\skewness}{\ensuremath{\zeta}}
\newcommand{\kurtosis}{\ensuremath{\kappa}}
\newcommand{\neff}{\ensuremath{N_{\rm eff}}}
\newcommand{\num}{\ensuremath{N}}
\newcommand{\nstd}{\ensuremath{\num_\sigma}}
\newcommand{\ndev}{\ensuremath{\num_{\rm dev}}}
\newcommand{\nstat}{\ensuremath{\num_{\rm stat}}}
\newcommand{\conflevel}{\ensuremath{\rm SL}}
\newcommand{\cov}{\ensuremath{\mathbf{C}}}
\newcommand{\tstat}{\ensuremath{\tau}}

% Bianchi
\newcommand{\bx}{\ensuremath{x}}
\newcommand{\bhand}{\ensuremath{\kappa}}
\newcommand{\bh}{\ensuremath{h}}
\newcommand{\ze}{\ensuremath{\zrec}}
\newcommand{\bshear}{\ensuremath{\left(\frac{\sigma}{H}\right)_0}}
\newcommand{\bsheardim}{\ensuremath{\sigma}}
\newcommand{\bshearonetwo}{\ensuremath{\left(\frac{\sigma_{12}}{H}\right)_0}}
\newcommand{\bshearonethree}{\ensuremath{\left(\frac{\sigma_{13}}{H}\right)_0}}
\newcommand{\bvort}{\ensuremath{\left(\frac{\omega}{H}\right)_0}}
\newcommand{\bshearinline}{\ensuremath{(\sigma/H)_0}}
\newcommand{\bvortinline}{\ensuremath{(\omega/H)_0}}
\newcommand{\ba}{\ensuremath{A}}
\newcommand{\bb}{\ensuremath{B}}
\newcommand{\bi}[2]{\ensuremath{I^{#1}_{#2}}}
\newcommand{\thetaph}{\ensuremath{\theta_0}}
\newcommand{\phiph}{\ensuremath{\phi_0}}
\newcommand{\thetaob}{\ensuremath{\theta_{\rm ob}}}
\newcommand{\phiob}{\ensuremath{\phi_{\rm ob}}}
\newcommand{\thetaalm}{\ensuremath{\theta}}
\newcommand{\phialm}{\ensuremath{\phi}}
\newcommand{\bs}{\ensuremath{s}}
\newcommand{\bt}{\ensuremath{\tau}}
\newcommand{\bps}{\ensuremath{\psi}}
\newcommand{\bcone}{\ensuremath{C_1}}
\newcommand{\bctwo}{\ensuremath{C_2}}
\newcommand{\bcthree}{\ensuremath{C_3}}
\newcommand{\alm}{\ensuremath{a}}
\newcommand{\almi}{\ensuremath{\shc{\alm}{\el}{\m}}}
\newcommand{\almpi}{\ensuremath{\shc{\alm}{\el}{\m\p}}}
\newcommand{\almitilde}{\ensuremath{\shc{\tilde{\alm}}{\el}{\m}}}

% Bianchi template fitting
\newcommand{\amptmpl}{\ensuremath{\lambda}}
\newcommand{\prob}{\ensuremath{{\rm P}}}
\newcommand{\given}{\ensuremath{{\,|\,}}}
\newcommand{\evidence}{\ensuremath{{E}}}
\newcommand{\param}{\ensuremath{\Theta}}
\newcommand{\bparam}{\ensuremath{\Theta_{\rm B}}}
\newcommand{\cosmoparam}{\ensuremath{\Theta_{\rm C}}}
\newcommand{\anisoparam}{\ensuremath{\Theta_{\rm A}}}
\newcommand{\fitdata}{\ensuremath{\vect{d}}}
\newcommand{\fitmodel}{\ensuremath{\vect{m}}}
\newcommand{\fitmodelsel}{\ensuremath{M}}
\newcommand{\fitamp}{\ensuremath{\lambda}}
\newcommand{\fitampest}{\ensuremath{\widehat{\lambda}}}
\newcommand{\fittmpl}{\ensuremath{\vect{b}}}
\newcommand{\fitnoise}{\ensuremath{\vect{n}}}
\newcommand{\fitcov}{\ensuremath{\mathbf{M}}}
\newcommand{\fitchisqd}{\ensuremath{\chi^2}}
\newcommand{\fitdatasky}{\ensuremath{d}}
\newcommand{\fitdataalm}{\ensuremath{\shc{d}{\el}{\m}}}
\newcommand{\fittmplalm}{\ensuremath{\shc{b}{\el}{\m}}}
\newcommand{\fitdataalz}{\ensuremath{\shc{d}{\el}{0}}}
\newcommand{\fittmplalz}{\ensuremath{\shc{b}{\el}{0}}}
\newcommand{\mnoise}{\ensuremath{m}}

% ISW/Cross-correlation
\newcommand{\wcov}{\ensuremath{X_\wav}}
\newcommand{\wcovest}{\ensuremath{\widehat{X}_\wav}}
\newcommand{\wcovvect}{\ensuremath{\mathbf{X}_\wav}}
\newcommand{\wcovestvect}{\ensuremath{\widehat{\mathbf{X}}_\wav}}
\newcommand{\covweight}{\ensuremath{\nu}}
\newcommand{\covsubterm}{\ensuremath{G^\el}}
\newcommand{\clnt}{\ensuremath{C_\el^{\rm NT, obs}}}
\newcommand{\clnttheo}{\ensuremath{C_\el^{\rm NT}}}
\newcommand{\clnntheo}{\ensuremath{C_\el^{\rm NN}}}
\newcommand{\cltttheo}{\ensuremath{C_\el^{\rm TT}}}
% \newcommand{\nd}{\ensuremath{N}}
% \newcommand{\tp}{\ensuremath{T}}
\newcommand{\ndlab}{\ensuremath{{\rm N}}}
\newcommand{\tplab}{\ensuremath{{\rm T}}}
\newcommand{\dndz}{\ensuremath{\frac{\dx N}{\dx z}}}
\newcommand{\dgdz}{\ensuremath{\frac{\dx g}{\dx z}}}
\newcommand{\eqdec}{\ensuremath{\delta}}
\newcommand{\chisqd}{\ensuremath{\chi^2}}
\newcommand{\baypar}{\ensuremath{\Theta}}
\newcommand{\lhood}{\ensuremath{\mathcal{L}}}

% Optimal filters
\newcommand{\fil}{\ensuremath{\varphi}}
\newcommand{\filcoeff}{\ensuremath{w}}
\newcommand{\lagrnmult}{\ensuremath{\mu}}
\newcommand{\lagrn}{\ensuremath{\mathcal{L}}}
\newcommand{\filvara}{\ensuremath{a}}
\newcommand{\filvarb}{\ensuremath{b}}
\newcommand{\filvarc}{\ensuremath{c}}
\newcommand{\filvardenom}{\ensuremath{\Delta}}
\newcommand{\pnorm}{\ensuremath{p}}
\newcommand{\pnormsep}{\ensuremath{|}}
\newcommand{\pnormtext}{\ensuremath{\pnorm}-norm}
\newcommand{\pnormtextit}{\ensuremath{\rm{\pnorm}}-norm}
\newcommand{\scalepnorm}{\ensuremath{{\scale\pnormsep\pnorm}}}
\newcommand{\scalenautpnorm}{\ensuremath{{\scalenaut\pnormsep\pnorm}}}
\newcommand{\za}[2]{\ensuremath{\shc{a}{#1}{#2}}}
\newcommand{\zb}[2]{\ensuremath{\shc{b}{#1}{#2}}}
\newcommand{\zc}[2]{\ensuremath{\shc{c}{#1}{#2}}}
\newcommand{\zd}[2]{\ensuremath{\shc{d}{#1}{#2}}}
\newcommand{\zcsp}[2]{\ensuremath{\shcsp{c}{#1}{#2}}}
\newcommand{\zdsp}[2]{\ensuremath{\shcsp{d}{#1}{#2}}}
\newcommand{\detect}{\ensuremath{\Gamma}}
\newcommand{\source}{\ensuremath{s}}
%\newcommand{\beam}{\ensuremath{b}}
\newcommand{\noise}{\ensuremath{n}}
\newcommand{\instnoise}{\ensuremath{r}}
\newcommand{\obsig}{\ensuremath{y}}
\newcommand{\conv}{\ensuremath{\star}}
\newcommand{\convdir}{\ensuremath{\circledast}}
\newcommand{\convaxisym}{\ensuremath{\odot}}
\newcommand{\amp}{\ensuremath{A}}
\newcommand{\tmpl}{\ensuremath{\tau}}
\newcommand{\noisecl}{\ensuremath{C}}
\newcommand{\amphat}{\ensuremath{\hat{A}}}
\newcommand{\eulshat}{\ensuremath{\hat{\alpha},\hat{\beta},\hat{\gamma}}}
\newcommand{\fconsta}{\ensuremath{A_{\el\pnorm}}}
\newcommand{\fconstb}{\ensuremath{B_{\el\m}}}

% Interferometry
\newcommand{\sao}{\ensuremath{\sa_0}}
\newcommand{\saog}{\ensuremath{\sao^{\glob}}}
\newcommand{\sag}{\ensuremath{\sa^{\glob}}}
\newcommand{\sal}{\ensuremath{\sa^{\loc}}}
\newcommand{\sae}{\ensuremath{\sa^{\erth}}}
\newcommand{\san}{\ensuremath{\sa^{\nght}}}
\newcommand{\saoe}{\ensuremath{\sao^{\erth}}}
\newcommand{\saon}{\ensuremath{\sao^{\nght}}}
\newcommand{\salcoordfree}{\ensuremath{\vect{\tau}}}
\newcommand{\vis}{\ensuremath{y}}
\newcommand{\visdis}{\ensuremath{\vect{y}}}
\newcommand{\beam}{\ensuremath{A}}
\newcommand{\beamp}{\ensuremath{A_{\pind}}}
\newcommand{\beams}{\ensuremath{A_{\sind}}}
\newcommand{\beamdis}{\ensuremath{\vect{\beam}}}
\newcommand{\im}{\ensuremath{x}}
\newcommand{\imdis}{\ensuremath{\vect{\im}}}
\newcommand{\noisedis}{\ensuremath{\vect{\noise}}}
\newcommand{\imp}{\ensuremath{\im_{\pind}}}
\newcommand{\ims}{\ensuremath{\im_{\sind}}}
\newcommand{\imm}{\ensuremath{\im_{\mind}}}
\newcommand{\nim}{\ensuremath{n}}
\newcommand{\visvect}{\ensuremath{\vect{\vis}}}
\newcommand{\imvect}{\ensuremath{\vect{\im}}}
\newcommand{\imvectrecon}{\ensuremath{\vect{\im}^{\star}}}
\newcommand{\impvect}{\ensuremath{\vect{\imp}}}
\newcommand{\imsvect}{\ensuremath{\vect{\ims}}}
\newcommand{\immvect}{\ensuremath{\imvect_{m}}}
\newcommand{\impvectrecon}{\ensuremath{\vect{\imp}^{\star}}}
\newcommand{\imsvectrecon}{\ensuremath{\vect{\ims}^{\star}}}
\newcommand{\nimvect}{\ensuremath{\vect{\nim}}}
\newcommand{\bu}{\ensuremath{u}}
\newcommand{\bv}{\ensuremath{v}}
\newcommand{\bw}{\ensuremath{w}}
\newcommand{\bwd}{\ensuremath{w_{\rm d}}}
\newcommand{\buvect}{\ensuremath{\vect{\bu}}}
\newcommand{\buvectfull}{\ensuremath{\vect{b}}}
\newcommand{\bumax}{\ensuremath{\bu_{\rm max}}}
\newcommand{\bumaxfov}{\ensuremath{\bumax}}
\newcommand{\elmaxfov}{\ensuremath{\elmax}}
\newcommand{\lx}{\ensuremath{l}}
\newcommand{\mx}{\ensuremath{m}}
\newcommand{\nx}{\ensuremath{n}}
\newcommand{\lxvect}{\ensuremath{\vect{\lx}}}
\newcommand{\lxvectdis}{\ensuremath{\vect{\lx}_{\ispar}}}
\newcommand{\blinel}{\ensuremath{\vect{u}}}
\newcommand{\blineg}{\ensuremath{\vect{u}^\glob}}
\newcommand{\blinee}{\ensuremath{\vect{u}^\erth}}
\newcommand{\inten}{\ensuremath{I}}
\newcommand{\loc}{\ensuremath{{\rm l}}}
\newcommand{\glob}{\ensuremath{{\rm n}}}
\newcommand{\erth}{\ensuremath{{\rm e}}}
\newcommand{\nght}{\ensuremath{{\rm n}}}
\newcommand{\beaml}{\ensuremath{\beam^\loc}}
\newcommand{\beamg}{\ensuremath{\beam^\glob}}
\newcommand{\intenl}{\ensuremath{\inten^\loc}}
\newcommand{\inteng}{\ensuremath{\inten^\glob}}
\newcommand{\intenn}{\ensuremath{\inten^\nght}}
\newcommand{\beammodintenl}{\ensuremath{\mbox{$\bigl( \beaml \cdot \intenl \bigr)$}}}
\newcommand{\beamhorzmodintenl}{\ensuremath{\mbox{$\bigl( \beaml \cdot \horizonl \cdot \intenl \bigr)$}}}
\newcommand{\blinemax}{\ensuremath{\|\vect{u}\|_{\rm max}}}
\newcommand{\horizon}{\ensuremath{H}}
\newcommand{\horizone}{\ensuremath{\horizon^\erth}}
\newcommand{\horizonl}{\ensuremath{\horizon^\loc}}
\newcommand{\chirp}{\ensuremath{C}}
\newcommand{\chirpfull}{\ensuremath{\chirp(\| \lxvect \|_2)}}
\newcommand{\chirpfulla}{\ensuremath{\chirp_{0}(\| \lxvect \|_2)}}
\newcommand{\chirpfullb}{\ensuremath{\chirp_{1}(\| \lxvect \|_2)}}
\newcommand{\chirpdis}{\ensuremath{\vect{\chirp}}}

\newcommand{\chirpfullbl}{\ensuremath{\bumax^{\chirp^{(\bw)}}}}
\newcommand{\chirpfullbbl}{\ensuremath{\bumax^{\chirp^{(\bw)}_1}}}

\newcommand{\expcoeff}{\ensuremath{E}}
\newcommand{\objsize}{\ensuremath{\sigma_{\rm S}}}
\newcommand{\plevel}{\ensuremath{p}}
\newcommand{\pfov}{\ensuremath{L}}

% Compressed sensing
\newcommand{\nmeas}{\ensuremath{M}}
\newcommand{\ndim}{\ensuremath{N}}
\newcommand{\sparsity}{\ensuremath{K}}
\newcommand{\ssmat}{\ensuremath{\Theta}}
\newcommand{\ispar}{\ensuremath{i}}
\newcommand{\isens}{\ensuremath{r}}
\newcommand{\sparatom}{\ensuremath{\vect{\psi}_\ispar}}
\newcommand{\sensatom}{\ensuremath{\vect{\phi}_\isens}}
\newcommand{\sparmat}{\ensuremath{\Psi}}
\newcommand{\sensmat}{\ensuremath{\Phi}}
\newcommand{\sensmatm}{\ensuremath{\Phi_{m}}}
\newcommand{\sensmatp}{\ensuremath{\Phi_{\pind}}}
\newcommand{\sensmats}{\ensuremath{\Phi_{\sind}}}
\newcommand{\coherence}{\ensuremath{\mu}}
\newcommand{\ccoherence}{\ensuremath{\nu}}
\newcommand{\coherences}{\ensuremath{\coherence _{\rm s}}}
\newcommand{\ccoherences}{\ensuremath{\ccoherence _{\rm s}}}
\newcommand{\coherencep}{\ensuremath{\coherence _{\rm p}}}
\newcommand{\ccoherencep}{\ensuremath{\ccoherence _{\rm p}}}

% Compressed sensing for interferometry
\newcommand{\opmask}{\ensuremath{\mathbfss{M}}}
\newcommand{\opbeam}{\ensuremath{\mathbfss{A}}}
\newcommand{\opfourier}{\ensuremath{\mathbfss{F}}}
\newcommand{\opwhite}{\ensuremath{\mathbfss{W}}}
\newcommand{\opchirp}{\ensuremath{\mathbfss{C}}}
\newcommand{\opgrid}{\ensuremath{\mathbfss{G}}}
\newcommand{\opproj}{\ensuremath{\mathbfss{P}}}

% Sparse signal reconstruction on the sphere
\newcommand{\opshtinv}{\ensuremath{\Lambda}}
\newcommand{\opshtfwd}{\ensuremath{\Gamma}}
\newcommand{\opshtcse}{\ensuremath{\Pi}}

% Bubble collisions
\newcommand{\thetacrit}{\ensuremath{\saa_{\rm crit}}}
\newcommand{\zo}{\ensuremath{z_{0}}}
\newcommand{\zcrit}{\ensuremath{z_{\rm crit}}}
\newcommand{\saao}{\ensuremath{\saa_{0}}}
\newcommand{\sabo}{\ensuremath{\sab_{0}}}
\newcommand{\saso}{\ensuremath{\saao, \sabo}}

% Cosmic strings
\newcommand{\gmu}{\ensuremath{G \mu}}
\newcommand{\fstring}{\ensuremath{s}}
\newcommand{\fcmb}{\ensuremath{c}}
\newcommand{\fdata}{\ensuremath{d}}
\newcommand{\fnoise}{\ensuremath{n}}
\newcommand{\fcmbnoise}{\ensuremath{{g}}}
\newcommand{\fstringrecov}{\ensuremath{\overline{\fstring}}}
\newcommand{\wcoeffstring}{\ensuremath{\wcoeff^\fstring}}
\newcommand{\wcoeffcmb}{\ensuremath{\wcoeff^\fcmb}}
\newcommand{\wcoeffdata}{\ensuremath{\wcoeff^\fdata}}
\newcommand{\wcoeffnoise}{\ensuremath{\wcoeff^\fnoise}}
\newcommand{\wcoeffcmbnoise}{\ensuremath{\wcoeff^{\fcmbnoise}}}
\newcommand{\wcoeffstringp}{\ensuremath{\wcoeffstring_{\wscaleposn}}}
\newcommand{\wcoeffcmbp}{\ensuremath{\wcoeffcmb_{\wscaleposn}}}
\newcommand{\wcoeffdatap}{\ensuremath{\wcoeffdata_{\wscaleposn}}}
\newcommand{\wcoeffnoisep}{\ensuremath{\wcoeffnoise_{\wscaleposn}}}
\newcommand{\wcoeffcmbnoisep}{\ensuremath{\wcoeffcmbnoise_{\wscaleposn}}}
\newcommand{\wcoeffstringprecov}{\ensuremath{\overline{\wcoeff}^\fstring_{\wscaleposn}}}
\newcommand{\wcoeffstringrecov}{\ensuremath{\overline{\wcoeff}^\fstring}}
\newcommand{\wvarcmb}{\ensuremath{(\sigma^\fcmb_\wscale)^2}}
\newcommand{\wstdcmb}{\ensuremath{\sigma^\fcmb_\wscale}}
\newcommand{\wvarstring}{(\sigma^\fstring_\wscale)^2}
\newcommand{\wstdstring}{\ensuremath{\sigma^\fstring_\wscale}}
\newcommand{\wkurstring}{\ensuremath{\kurtosis^\fstring_\wscale}}
\newcommand{\ggdshape}{\ensuremath{\changed{\xi}}}
\newcommand{\ggdscale}{\ensuremath{\changed{\zeta}}}
\newcommand{\ggdshapew}{\ensuremath{{\ggdshape_\wscale}}}
\newcommand{\ggdscalew}{\ensuremath{{\ggdscale_\wscale}}}
\newcommand{\modelstring}{\ensuremath{{{\rm M}^{\rm \fstring}}}}
\newcommand{\modelcmb}{\ensuremath{{{\rm M}^{\rm \fcmb}}}}

% Weak lensing
\newcommand{\wlconv}{\ensuremath{\prescript{}{0}{\kappa}}}
\newcommand{\wlshear}{\ensuremath{\prescript{}{2}{\gamma}}}
\newcommand{\wlshearone}{\ensuremath{\gamma_1}}
\newcommand{\wlsheartwo}{\ensuremath{\gamma_2}}
\newcommand{\wlpot}{\ensuremath{\prescript{}{0}{\phi}}}

\newcommand{\wlconvshc}{\ensuremath{\sshc{\hat{\kappa}}{\el}{\m}{0}}}
\newcommand{\wlshearshc}{\ensuremath{\sshc{\hat{\gamma}}{\el}{\m}{2}}}
\newcommand{\wlpotshc}{\ensuremath{\sshc{\hat{\phi}}{\el}{\m}{0}}}

\newcommand{\wlconvf}{\ensuremath{\prescript{}{0}{\hat{\kappa}}}}
\newcommand{\wlshearf}{\ensuremath{{\hat{\gamma}_1}}}
\newcommand{\wlshearonef}{\ensuremath{{\hat{\gamma}_1}}}
\newcommand{\wlsheartwof}{\ensuremath{{\hat{\gamma}_2}}}
\newcommand{\wlpotf}{\ensuremath{\prescript{}{0}{\hat{\phi}}}}

\newcommand{\wlconvfk}{\ensuremath{\prescript{}{0}{\hat{\kappa}(\wlkx,\wlky)}}}
\newcommand{\wlshearfk}{\ensuremath{\prescript{}{2}{\hat{\gamma}(\wlkx,\wlky)}}}
\newcommand{\wlshearonefk}{\ensuremath{{\hat{\gamma}_1(\wlkx,\wlky)}}}
\newcommand{\wlsheartwofk}{\ensuremath{{\hat{\gamma}_2(\wlkx,\wlky)}}}
\newcommand{\wlpotfk}{\ensuremath{\prescript{}{0}{\hat{\phi}(\wlkx,\wlky)}}}

\newcommand{\wlkx}{\ensuremath{k_x}}
\newcommand{\wlky}{\ensuremath{k_y}}

\newcommand{\wlfactor}{\ensuremath{\mathcal{D}}}
\newcommand{\wlfactorplane}{\ensuremath{\mathcal{E}}}
\newcommand{\wlkernel}{\ensuremath{\prescript{}{2}{\mathcal{K}}}}


